Mitigating TLS compromise with ECDHE and SRP

The paper reviews an implementation of an additional encrypted tunnel within TLS to further secure and authenticate the traffic of personal information between ProtonMail's frontends and the backend, implementing its key exchange, symmetric packet encryption, and validation. Technologies such as Secure Remote Password (SRP) and the Elliptic Curves Diffie Hellman Ephemeral (ECDHE) exchange are used for the key exchange, verifying the public parameters through PGP signatures. The data is then transferred encrypted with AES-128-GCM. This project is meant to integrate TLS security for high security data transfer, offering a flexible model that is easy to implement in the frontends by reusing part of the standard already existing in the PGP libraries.

==> commands.tex <==
\makeatletter
% case 1: theorem name--number ("ordinary") style
\patchcmd{\thmhead@plain}%
   {\thmnote{ {\the\thm@notefont(#3)}}}%  original form
   {\thmnote{:  #3}}%  new form
   {}{}
\let\thmhead\thmhead@plain

%\renewcommand{\qed}{\hfill \ensuremath{\Box}}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\newcommand\sigmaeq{\stackrel{\mathclap{\normalfont\mbox{$\sigma$-add}}}{\quad=\quad}}
\newcommand\aceq{\stackrel{\mathclap{\normalfont\mbox{qc}}}{\;=\;}}
\newcommand{\indep}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}
\newcommand{\padtwo}[1]{\ifnum #1 < 10 0\fi #1}

\newenvironment{dedication}
  {\clearpage           % we want a new page
   \thispagestyle{empty}% no header and footer
   \vspace*{\stretch{1}}% some space at the top
   \itshape             % the text is in italics
   \raggedleft          % flush to the right margin
  }
  {\par % end the paragraph
   \vspace{\stretch{2}} % space at bottom is three times that at the top
   \clearpage     % finish off the page
  }

\newcommand*{\blankpage}{%

}

%cleardoublepage lascia le pagine bianche, con solo il numero
\makeatletter
\def\emptypage@emptypage{%
    \hbox{}%
    \thispagestyle{plain}   %% or any page style
    \blankpage%
    \newpage%
}%
\def\cleardoublepage{%
        \clearpage%
        \if@twoside%
            \ifodd\c@page%
                % do nothing
            \else%
                \emptypage@emptypage%
            \fi%
        \fi%
    }%
\makeatother

% SCORCIATOIE PERSONALIZZATE

%% Formattazione
\newcommand{\Fixvmode}{\leavevmode\vspace{-\baselineskip}}

\newcommand{\DoCo}[1][n]{(\Omega, \Ac, \PP) \to \ifthenelse{\equal{#1}{1}}{(\RR, \Bc)}{(\RR^{#1}, \Bc^{#1})}}
\newcommand{\Dom}{(\Omega, \Ac, \PP)}
\newcommand{\Ex}[1]{\EE \left[ #1 \right]}
\newcommand{\IS}{È }
\newcommand{\notindep}{\centernot{\indep}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\markov}{\operatorname{Markov}}
\renewcommand{\H}{\operatorname{Hash}}

%Lettere fighe/corsive
\newcommand{\Ac}{\mathcal A}
\newcommand{\Bc}{\mathcal B}
\newcommand{\Cc}{\mathcal C}
\newcommand{\Dc}{\mathcal D}
\newcommand{\Ec}{\mathcal E}
\newcommand{\Fc}{\mathcal F}
\newcommand{\Gc}{\mathcal G}
\newcommand{\Hc}{\mathcal H}
\newcommand{\Ic}{\mathcal I}
\newcommand{\Jc}{\mathcal J}
\newcommand{\Kc}{\mathcal K}
\newcommand{\Lc}{\mathcal L}
\newcommand{\Mc}{\mathcal M}
\newcommand{\mm}{\mathscr m} %per la misura di Lebesgue
\newcommand{\Nc}{\mathcal N}
\newcommand{\Oc}{\mathcal O}
\newcommand{\Pc}{\mathcal P}
\newcommand{\Qc}{\mathcal Q}
\newcommand{\Rc}{\mathcal R}
\newcommand{\Sc}{\mathcal S}
\newcommand{\Tc}{\mathcal T}
\newcommand{\Uc}{\mathcal U}
\newcommand{\Vc}{\mathcal V}
\newcommand{\Wc}{\mathcal W}
\newcommand{\Xc}{\mathcal X}
\newcommand{\Yc}{\mathcal Y}
\newcommand{\Zc}{\mathcal Z}

%% Doppia barra
\renewcommand{\AA}{\mathbb A}
\newcommand{\BB}{\mathbb B}
\newcommand{\CC}{\mathbb C}
\newcommand{\DD}{\mathbb D}
\newcommand{\EE}{\mathbb E}
\newcommand{\FF}{\mathbb F}
\newcommand{\GG}{\mathbb G}
\newcommand{\HH}{\mathbb H}
\newcommand{\II}{\mathbb I}
\newcommand{\JJ}{\mathbb J}
\newcommand{\KK}{\mathbb K}
\newcommand{\LL}{\mathbb L}
\newcommand{\MM}{\mathbb M}
\newcommand{\NN}{\mathbb N}
\newcommand{\OO}{\mathbb O}
\newcommand{\PP}{\mathbb P}
\newcommand{\QQ}{\mathbb Q}
\newcommand{\RR}{\mathbb R}
\renewcommand{\SS}{\mathbb S}
\newcommand{\TT}{\mathbb T}
\newcommand{\UU}{\mathbb U}
\newcommand{\VV}{\mathbb V}
\newcommand{\WW}{\mathbb W}
\newcommand{\XX}{\mathbb X}
\newcommand{\YY}{\mathbb Y}
\newcommand{\ZZ}{\mathbb Z}

% d nell'integrale
\newcommand{\de}{\mathrm d}
\newcommand{\dx}{\de x}
\newcommand{\dy}{\de y}
\newcommand{\dP}{\de P}
\newcommand{\dPP}{\de \PP}

% \bigcdot un pallino per le var nelle funzioni
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\usetikzlibrary{patterns}
\makeatletter
\pgfdeclarepatternformonly[\hatchdistance,\hatchthickness]{flexible hatch}
  {\pgfqpoint{0pt}{0pt}}
  {\pgfqpoint{\hatchdistance}{\hatchdistance}}
  {\pgfpoint{\hatchdistance-1pt}{\hatchdistance-1pt}}%
  {
      \pgfsetcolor{\tikz@pattern@color}
      \pgfsetlinewidth{\hatchthickness}
      \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
      \pgfpathlineto{\pgfqpoint{\hatchdistance}{\hatchdistance}}
      \pgfusepath{stroke}
  }
\makeatother

% Indice su 2 colonne
%\makeindex[columns=2]

% Padding verticale nelle celle
% uso: \CS[spazio sopra]{spazio sotto}
%\newcommand{\CS}[2][0]{\rule{0pt}{#1 cm} \rule[-#2cm]{0pt}{0pt}}


==> imp/introduction.tex <==
In this chapter the practical problem is going to be analyzed, to understand the \textit{threat model}; then the tunnel stucture, first schematically then server and client-side implementation.

